Stability of Quantum Computers

Quantum computing's potential is immense, promising super-polynomial reductions in execution time, energy use, and memory requirements compared to classical computers. This technology has the power to revolutionize scientific applications such as simulating many-body quantum systems for molecular structure understanding, factorization of large integers, enhance machine learning, and in the process, disrupt industries like telecommunications, material science, pharmaceuticals and artificial intelligence. However, quantum computing's potential is curtailed by noise, further complicated by non-stationary noise parameter distributions across time and qubits. This dissertation focuses on the persistent issue of noise in quantum computing, particularly non-stationarity of noise parameters in transmon processors.

==> back-matter/vita.tex <==
\chapter*{Vita}\label{ch:vita}
Samudra Dasgupta completed his Bachelor of Technology in Electronics and Electrical Communications Engineering from the Indian Institute of Technology, Kharagpur, where he won the best undergraduate thesis award for his work demonstrating the constructive use of noise in SNR (signal-to-noise raio) enhancement. He obtained his Master of Science in Engineering  Sciences from Harvard University, Cambridge.

==> chapters/hamiltonian_vqe.tex <==
\section{Hamiltonian}
\subsection{What is the role of the Hamiltonian operator in quantum mechanics?}
The Hamiltonian operator provides a mathematical description of the system's energy and determines how it changes over time. It acts on wave functions to yield the corresponding energy values. The eigenvalues of the Hamiltonian operator correspond to the allowed energy levels of the system, while the corresponding eigenvectors (wave functions) represent the states associated with those energy levels. The Hamiltonian operator encapsulates various physical quantities and interactions within a quantum system. It includes terms related to the system's kinetic energy, potential energy, and any interactions with external fields or other particles. This makes it a crucial component in studying and analyzing the behavior of quantum systems, as it provides insights into the system's energy spectrum and dynamics.

\subsection{How does the Hamiltonian operator relate to the energy of a quantum system?}
The Hamiltonian operator is directly related to the energy of a quantum system. In quantum mechanics, the energy of a system is determined by the eigenvalues of the Hamiltonian operator. When the Hamiltonian operator acts on a quantum state (represented by a wave function), it yields a new state that is proportional to the original state. This proportionality factor is the energy associated with the state, and it is given by the eigenvalue of the Hamiltonian operator for that particular state. Mathematically, if we have a quantum state represented by a wave function $\ket{\Psi}$, the action of the Hamiltonian operator (denoted as H) on $\ket{\Psi}$ can be expressed as:

\[ H\ket{\Psi} = \ket{\Psi}\],

where E represents the energy associated with the state $\ket{\Psi}$, and it is an eigenvalue of the Hamiltonian operator. In this context, the Hamiltonian operator serves as an observable in quantum mechanics. When we measure the energy of a quantum system, we are essentially determining the eigenvalues of the Hamiltonian operator for the corresponding states. By solving the eigenvalue problem for the Hamiltonian operator, we can determine the set of allowed energy levels and their associated eigenstates (wave functions) for a given quantum system. These energy eigenstates provide information about the possible energy values that the system can possess. In summary, the Hamiltonian operator directly relates to the energy of a quantum system. Its eigenvalues correspond to the possible energy levels of the system, and the associated eigenstates represent the states with those energy levels. The Hamiltonian operator allows us to quantify and analyze the energy spectrum of quantum systems, providing crucial information about their physical behavior.

\subsection{What is the link between the Hamiltonian and quantum dynamics?}
In quantum mechanics, the time evolution of a quantum state is described by the Schrödinger equation. The Schrödinger equation relates the time derivative of the quantum state to the Hamiltonian operator. It can be written as:

\[ i\bar{h} \frac{\partial \ket{\Psi}}{\partial t} = H \ket{\Psi}, \]

This equation essentially states that the rate of change of the quantum state with respect to time is proportional to the action of the Hamiltonian operator on that state. It establishes a direct relationship between the Hamiltonian operator and the dynamics of the quantum system. By solving the Schrödinger equation, one can obtain the time-dependent wave function, which describes how the quantum state of the system evolves over time. The Hamiltonian operator determines the specific form and behavior of the time evolution. The eigenstates (energy eigenstates) of the Hamiltonian operator play a critical role in the time evolution of quantum systems. These eigenstates form a complete set, which means any quantum state can be expressed as a linear combination of the eigenstates. As time progresses, the coefficients of these eigenstates may change, resulting in the evolution of the quantum state. The Hamiltonian operator also accounts for the energy transfer and transformations within the system. It incorporates terms related to the kinetic energy, potential energy, and any interactions present. These terms influence how the quantum system evolves and how its energy changes over time.

\subsection{What does the Hamiltonian operator govern in terms of the time evolution of a quantum system?}
The Hamiltonian operator encompasses various terms that contribute to the energy and dynamics of the quantum system. It includes components related to the kinetic energy of particles, potential energy arising from interactions within the system or with external fields, and any other relevant energy contributions. The Hamiltonian operator determines the energy dynamics, energy transfer, and transformations within the system as it governs the time-dependent changes in the quantum state.

\subsection{What kind of questions does the Hamiltonian formalism does not help answer?}
There are certain types of questions that the Hamiltonian formalism may not directly answer or may not be well-suited for. Here are some examples:\\
1. Measurement Outcomes: The Hamiltonian formalism primarily focuses on the time evolution and energy spectrum of quantum states. It does not provide explicit predictions for measurement outcomes or probabilities associated with specific measurement results. To obtain measurement probabilities and specific outcomes, one typically needs to consider additional postulates, such as those provided by the Copenhagen interpretation or the measurement theory in quantum mechanics.\\
2. Observable Values: While the Hamiltonian operator represents an observable associated with the energy of a system, it may not directly provide information about other observables. Observables other than energy, such as position or momentum, may require different operators or formalisms to analyze and extract information about their values and measurements.\\
3. Entanglement Properties: The Hamiltonian formalism can describe entangled states, but it may not explicitly provide information about the entanglement properties of a system or the specific correlations between entangled particles. The study of entanglement typically involves other formalisms, such as density matrices or entanglement measures, to quantify and analyze the entanglement present in a given state.\\
4. Decoherence and Environmental Interactions: The Hamiltonian formalism assumes an isolated quantum system. It does not explicitly address the effects of environmental interactions or decoherence, which can cause loss of coherence and entanglement in real-world quantum systems. To analyze and understand these effects, additional techniques, such as open quantum systems or master equations, are often employed.\\
5. Interpretational Questions: The Hamiltonian formalism, as a mathematical framework, does not provide definitive answers to interpretational questions in quantum mechanics, such as the nature of wave function collapse or the interpretation of quantum superposition. Interpretational questions often involve philosophical or conceptual discussions that go beyond the mathematical formalism itself.
    
\subsection{Why is it hard to simulate the Hamiltonian of a many body system?}
Simulating the time evolution governed by the Hamiltonian, such as solving the Schrödinger equation, can become computationally expensive for many-body systems.\\

The dimensionality of the Hilbert space grows exponentially with the number of particles in the system. For a system of N particles, the dimension of the Hilbert space is $2^N$.\\

The exponential growth in the dimensionality of the Hilbert space leads to substantial memory and computational requirements.\\

Many-body systems often exhibit strong quantum correlations and entanglement between particles. As the number of particles increases, the entanglement grows, leading to complex and non-local interactions in the system. Capturing and representing these correlations accurately becomes increasingly difficult.\\

Many-body systems often involve interactions between particles that can be long-range or depend on the distance between particles. Modeling and simulating these interactions accurately can introduce additional computational challenges and complexities.\\

Due to these challenges, simulating the Hamiltonian of a many-body system often requires the development and application of specialized techniques, such as quantum Monte Carlo methods, tensor network methods, or variational approaches. These methods aim to exploit the specific properties and structures of the Hamiltonian to efficiently approximate or simulate the behavior of the system.\\

\subsection{Why is it hard to simulate the Hamiltonian of a topological quantum state?}
Simulating the Hamiltonian of a topological quantum state can be challenging due to several reasons:
\begin{itemize}
\item Topological Protection: Topological quantum states are known for their robustness against certain types of perturbations. This protection arises from non-local properties and long-range entanglement within the system. Simulating the Hamiltonian of a topological state requires capturing these non-local features accurately, which can be computationally demanding.

\item Ground State Degeneracy: Many topological quantum states exhibit ground state degeneracy, meaning they have multiple degenerate ground states with different topological properties. Simulating the Hamiltonian to capture and distinguish these different ground states can be challenging, as it requires maintaining and manipulating multiple states simultaneously.

\item Non-Local Correlations: Topological quantum states often exhibit long-range entanglement and non-local correlations, which can extend over large distances within the system. Capturing and representing these non-local correlations accurately in a simulation can be computationally expensive and require sophisticated techniques, such as tensor network methods or entanglement renormalization.

\item Large System Sizes: Topological quantum states can arise in systems with a large number of particles or degrees of freedom. The simulation of such large systems becomes increasingly challenging due to the exponential growth in the size of the Hilbert space and the computational resources required to represent and manipulate the associated Hamiltonian.

\item Sparse Matrix Structure: The Hamiltonians describing topological quantum states often have a sparse matrix structure, with a pattern of non-zero elements that may be complex and system-dependent. Efficient storage and manipulation of the sparse Hamiltonian matrix can be computationally demanding, especially for large systems.

\item Emergent Phenomena: Topological quantum states can exhibit emergent phenomena that are not apparent at the microscopic level. Simulating these emergent behaviors and capturing their properties in a simulation can be challenging, as they may involve collective behavior of many particles or interactions that are difficult to model accurately.

One prominent example of emergent phenomena in topological quantum states is the phenomenon of anyons. Anyons are quasiparticles that can emerge in certain two-dimensional topological quantum systems. In two-dimensional topological systems, particles can exhibit fractional statistics, which means their exchange statistics are neither purely bosonic (exchanging two identical bosons leads to no change) nor purely fermionic (exchanging two identical fermions leads to a sign change in the wave function). Instead, anyons have fractional exchange statistics that can be anyonic, leading to non-trivial braiding properties. An example of a topological quantum state that exhibits anyons is the fractional quantum Hall effect (FQHE). In a two-dimensional electron gas subject to a strong magnetic field, under certain conditions, electrons can form a topologically ordered state. In this state, excitations occur with fractional charges and obey fractional statistics, giving rise to anyonic quasiparticles called "Laughlin quasiparticles." These anyons have properties that are distinct from familiar fermions or bosons. The emergent phenomena associated with anyons in the FQHE include:

1. \textbf{Fractional Charges}: Anyons in the FQHE carry fractional electric charges, which are fractions of the elementary charge. These fractional charges are not seen in conventional particles and emerge due to the collective behavior of electrons in the topological state.

2. \textbf{Braiding Statistics}: Anyons exhibit non-trivial braiding statistics, which means that when anyons are exchanged, their wave function acquires a non-trivial phase factor. This exchange of anyons can be harnessed to perform topological quantum computations using braiding operations.

3. \textbf{Topological Order}: The FQHE exhibits topological order, where the ground state has long-range entanglement and non-local correlations that are robust against local perturbations. This topological order is an emergent property that arises due to the collective behavior of many electrons in the system.

These emergent phenomena in the FQHE are a result of the unique properties of the topological quantum state and the interactions between particles. They are not present in the individual electrons but emerge at the macroscopic scale due to the collective behavior and topological properties of the system. The study of anyons and emergent phenomena in topological quantum states is an active area of research with implications for both fundamental physics and potential applications in topological quantum computation and fault-tolerant quantum information processing.

\end{itemize}

\subsection{How can you simulate the hamiltonian of a topological quantum state with noise using qiskit?}
See here: https://medium.com/qiskit/simulating-topological-systems-with-qiskit-pulse-9afac342ab09

\subsection{How is the Hamiltonian operator applied in different areas of quantum physics, such as quantum chemistry, solid-state physics, and particle physics?}

Here's how the Hamiltonian operator is applied:
\begin{itemize}
\item Quantum Chemistry: In quantum chemistry, the Hamiltonian operator is used to describe the behavior of electrons in molecules and atoms. It includes terms for the kinetic energy of electrons, the electron-electron interactions (Coulombic repulsion), and the electron-nucleus interactions. By solving the Schrödinger equation with the Hamiltonian operator, quantum chemists can obtain the electronic wave functions and energy levels of molecules. This information is crucial for understanding chemical bonding, molecular properties, spectroscopy, and chemical reactions.

\item Solid-State Physics: In solid-state physics, the Hamiltonian operator is used to describe the behavior of electrons in crystalline solids. The Hamiltonian includes terms for the kinetic energy of electrons in the crystal lattice, the electron-electron interactions, and the electron-lattice interactions (such as electron-phonon interactions). Solving the Schrödinger equation with the Hamiltonian operator allows physicists to study the electronic band structure, electrical conductivity, magnetism, and other properties of solid materials. This knowledge is essential for understanding the behavior of semiconductors, metals, insulators, and other condensed matter systems.

\item Particle Physics: In particle physics, the Hamiltonian operator is used to describe the behavior of elementary particles and their interactions. The Hamiltonian includes terms for the kinetic energy of particles, their interactions through fundamental forces (such as electromagnetic, weak, and strong forces), and possible interactions with external fields. By solving the Schrödinger or Dirac equation with the Hamiltonian operator, physicists can study particle interactions, particle decays, particle production, and other phenomena in particle accelerators and cosmic-ray experiments. This enables the exploration of the fundamental particles and their properties, leading to insights into the fundamental forces and the nature of matter.
underlying physics.
\end{itemize}


\section{VQE}
The ground state energy of a molecule refers to the lowest possible energy level that the molecule can have when it is in its most stable configuration, which is typically the state in which the electrons are distributed among the atoms in the molecule in the most energetically favorable way. It is determined by solving the Schrödinger equation for the molecule and is expressed in terms of the total energy of the electrons and the nuclei that make up the molecule. It provides a reference point for understanding the electronic and chemical properties of a molecule. Changes in the ground state energy due to chemical reactions or external influences can affect a molecule's reactivity, stability, and other properties.

For example, the ground state energy of water is -2.798 Hartree per molecule. % while that of diamond is approximately -0.270 Hartree per atom.
This means that -2.798 Hartree (1 Hartree = 27.2114 eV) of energy must be added to the water molecule to bring it to its unbound, or dissociated, state in which the constituent atoms and electrons are completely separated from each other (i.e. at infinity). Note that these values are approximate and may differ depending on the specific computational method and level of theory used to calculate them.

An accurate knowledge of the ground state energy of molecules has many practical applications e.g.
\begin{itemize}
\item Predicting chemical reactivity: The ground state energy of a molecule provides important information about its stability and reactivity. By comparing the ground state energies of different molecules, chemists can predict which reactions are likely to occur and design new molecules with specific properties.
\item Designing new materials: The ground state energy of a material is related to its electronic and structural properties, such as its band gap, electronic conductivity, and mechanical strength. Materials scientists use this information to design new materials with specific properties for applications such as solar cells, batteries, and catalysts.
\item Studying biological molecules: The ground state energy of a protein or nucleic acid molecule is closely related to its structure and function. Biophysicists use this information to study the folding and dynamics of biological molecules, which is important for understanding how they interact with other molecules and carry out their biological functions.
\item Analyzing spectroscopic data: The ground state energy of a molecule is related to its vibrational and rotational modes, which can be probed using various spectroscopic techniques, such as infrared spectroscopy and Raman spectroscopy. By analyzing the spectral data, chemists and physicists can determine the molecular structure and study the interactions between molecules.
\end{itemize}

However, it is very hard to determine the ground state energy of molecules accurately. There are many reasons for this difficulty. Firstly, it is a "many-body" problem, which is notoriously difficult to solve analytically, even without introducing quantum mechanics. Secondly, the quantum-mechanical wave function of a molecule (needed to find the ground state energy) becomes more and more complex as the size and geometrical intricacy of a molecule increases. As a result, even with modern supercomputers, the calculations can be computationally intensive and time-consuming, as it requires the evaluation of many integrals and the solution of large matrices. To simplify the problem, quantum chemists often make various approximations and assumptions when calculating the ground state energy of molecules. However, these approximations can introduce errors and uncertainties in the results. Despite these challenges, there have been significant advances in computational methods and algorithms for calculating the ground state energy of molecules, and researchers continue to develop new techniques to improve the accuracy and efficiency of these calculations.

Currently, the ground state energy of molecules is computed using four types of computational methods. The first is the density functional theory (DFT) that approximates the electron density of a molecule or material, rather than the full wave function. It is the least accurate but highly scaleable. The second commonly used method is the Hartree-Fock (HF) method which is used for small and medium-sized molecules. It uses a single Slater determinant wave function (which is an approximation to the true wave function of the molecule because it assumes that the electrons in the molecule are non-interacting), to describe the electronic structure of a molecule. The third commonly used method is the coupled cluster (CC) method which uses a truncated series of wave functions to describe the electronic structure of a molecule. In this method, the wave functions are constructed by applying a cluster operator (describing the correlation between the electrons in the molecule) to the Hartree-Fock (HF) wave function and expanding it in a power series. It is more computationally demanding than DFT and HF, but it can provide highly accurate results for small and medium-sized molecules. Lastly, we have the Quantum Monte Carlo (QMC) method which uses random sampling to solve the Schrödinger equation and compute the ground state energy of a molecule. It can provide highly accurate results for both small and large molecules, but it is computationally demanding and requires a significant amount of computational resources.

VQE (Variational Quantum Eigensolver) is a promising quantum algorithm for calculating the ground state energy of molecules and materials. It is designed to be run on a quantum computer, which is expected to be more efficient for certain types of calculations than classical computers. It uses quantum circuits to prepare trial wave functions, which are quantum states that represent the electronic structure of a molecule or material. This approach is believed to be more efficient for certain types of calculations, such as finding the ground state energy of large and complex molecules, compared to other methods that rely on approximations or perturbative expansions. Moreover, VQE is a flexible and scalable method that can be adapted to different types of problems and hardware architectures. Although VQE promises to find the ground state of systems that are too large for classical methods to handle and with higher accuracy, its advantage over classical methods for large molecules is yet to be demonstrated as current quantum computers are too small and noisy. 

\subsection{Method in brief}
VQE is a variational method. It is a hybrid quantum-classical algorithm. It simulates a molecule for finding its ground State energy. The method is as follows:\\

\begin{itemize}
    \item Input: Hamiltonian e.g. 
\begin{equation}
H = 32 I_0 -2 X_1 -2 Z_0 X_1 + 17 Z_1 + 3 X_0 Z_1 -23 Z_0 Z_1 -3 X_0 -26 Z_0
\end{equation}

\item Process: create a wave function ansatz of the molecule and calculate the expectation value using the Hamiltonian. (An An ansatz is a quantum state prepared using a parameterized quantum circuit.  Ansatz design not easy because it should be fairly complex and yet optimization of parameters should be quick.)

\item Output (examples): a) ground state energy b) dissociation curve i.e. plot of how the ground state energy varies with the distance between atoms in the molecule.
\end{itemize}


==> chapters/literature_review.tex <==
\section{Bayesian Learning in Quantum Computing}
\begin{enumerate}
\item arXiv:2204.05757\\
Dealing with quantum computer readout noise through high energy physics unfolding methods\\
This paper shows how to mitigate readout noise using Iterative Bayesian Unfolding (IBU) - a method that traces its roots to high energy physics. It has the advantage of avoiding the problem of unphysical outcomes and/or oscillatory behavior displayed by matrix inversion and least-squares. They generated.

\item arXiv:2203.13848\\
Optimal quantum kernels for small data classification\\
This paper shows a Bayesian algorithm for constructing quantum kernels that adapts quantum gate sequences to data. Using a Bayesian information metric, it performs a greedy search to select an optimal circuit in the space of quantum circuits and further uses Bayesian techniques to optimize the circuit parameters. The use-case is a classification problem with a small number of training points.

\item arXiv:2203.02464\\
Surviving The Barren Plateau in Variational Quantum Circuits with Bayesian Learning Initialization\\
The classical part of variational hybrid algorithms are computationally intensive due to the barren plateau phenomenon in parameterized quantum circuits. In this paper, the authors use Bayesian Learning instead to identify a promising region in parameter space that initializes a fast local optimizer to find the global optimum point more efficiently. They illustrate the method using a quantum generative model.

\item arXiv:2202.10601\\
Quantum Gaussian process model of potential energy surface for a polyatomic molecule\\
In this paper, the authors study the modeling of potential-energy-surface for molecules. The output is a Gaussian process regression model. They use Bayesian Learning to optimize circuit parameters. The basic idea is that quantum state projections can produce kernels of reproducing kernel Hilbert spaces. 

\item arXiv:2112.02025\\
Observing ground-state properties of the Fermi-Hubbard model using a scalable algorithm on a quantum computer\\
This paper implements a low-depth variational algorithm for a medium-size instance of the Fermi-Hubbard model (note that large scale models of these strongly-correlated electronic systems are beyond NISQ reach). It reproduces important qualitative features in the ground-state such as the onset of the metal-insulator transition and Friedel oscillations in 1D. The algorithm uses iterative Bayesian updates.  

\item arXiv:2112.00426\\
Noisy Bayesian optimization for variational quantum eigensolvers\\
This work proposes an implementation of Gaussian process regression and Bayesian optimization specifically tailored to perform the variational quantum eigensolver to study lattice gauge theories in the Hamiltonian formulation, with a very low number of iterations using data affected by statistical noise. 

\item arXiv:2109.05314\\
JigSaw: Boosting Fidelity of NISQ Programs via Measurement Subsetting\\
This work deploys Bayesian post-processing to update the histogram produced by the full-circuit using histograms produced by measuring a subset of the output qubits. 

\item arXiv:2108.10686\\
Experimental Bayesian estimation of quantum state preparation, measurement, and gate errors in multi-qubit devices\\
In this work, the authors use Bayesian methods for estimating single qubit errors (state preparation, readout, and gate) errors and study the stability of these errors as a function of time. They also demonstrate easily implemented mitigation approaches. They are able to resolve small parameters with a high relative accuracy, at a lower measurement cost as compared with standard characterization approaches. 

\item arXiv:2107.14473\\
Fast Bayesian tomography of a two-qubit gate set in silicon\\
In this work, the authors use bayesian techniques to perform self-consistent process tomography. Their algorithm can leverage prior information from randomised benchmarking and can be performed in real time (i.e. can provide continuously updated estimates of full process matrices while data is acquired). 

\item arXiv:2106.06113\\
Sample-efficient adaptive calibration of quantum networks using Bayesian optimization\\
Indistinguishable photons are imperative for distributed quantum computing, communications, and sensing, as well as for fundamental investigations. In this work, the authors develop a sample-efficient adaptive methodology to calibrate the indistinguishability of individual photons. It is fast, resource-optimized and experimentally friendly. It uses Bayesian optimization to adaptively calibrate the indistinguishability of individual photons for quantum networks using only information derived from their measurement in the presence of high loss and shot noise. 

\item arXiv:2105.05018\\
Optimizing the Phase Estimation Algorithm Applied to the Quantum Simulation of Heisenberg-Type Hamiltonians\\
This work uses Bayesian techniques to optimize the phase estimation algorithm (used in cryptography, number theory, and simulation of quantum systems) to simulate the time evolution of a system of two spin-1/2 particles under a Heisenberg Hamiltonian.

\item arXiv:2103.06720\\
Variational inference with a quantum computer\\
Inference is the task of drawing conclusions about unobserved variables given observations of related variables. Unfortunately, performing exact inference is intractable in general. One alternative is variational inference, where a candidate probability distribution is optimized to approximate the posterior distribution over unobserved variables. For good approximations, a flexible and highly expressive candidate distribution is desirable. In this work, the authors use quantum Born machines as variational distributions over discrete variables. They apply the framework of operator variational inference to achieve this goal. In particular, they adopt two specific realizations: one with an adversarial objective and one based on the kernelized Stein discrepancy. They demonstrate the approach numerically using examples of Bayesian networks, and implement an experiment on an IBM quantum computer. Their techniques enable efficient variational inference with distributions beyond those that are efficiently representable on a classical computer.

\item arXiv:2010.09075\\
Bayesian Quantum Multiphase Estimation Algorithm\\
This paper implements a Bayesian algorithm for the parallel (simultaneous) estimation of multiple arbitrary phases. The protocol gives access to correlations.

\item arXiv:2010.09188\\
A Bayesian Approach for Characterizing and Mitigating Gate and Measurement Errors\\

\item arXiv:2006.09350\\
Minimizing estimation runtime on noisy quantum computers\\
Used Bayesian inference to enhance the power of sampling on noisy quantum devices. Reduces measurement number and runtime compared to the standard sampling method of VQE. Enhances the rate of information gain in sampling as the physical hardware transitions from NISQ ti QECC.

\item arXiv:2004.01992\\
A hidden variable model for universal quantum computation with magic states on qubits \\
Authors show that every quantum computation can be described by Bayesian update of a probability distribution on a finite state space.

\item arXiv:1912.10857\\
Bayesian machine learning for Boltzmann machine in quantum-enhanced feature spaces\\
Authors propose the quantum bayesian learning framework of the restricted Boltzmann machine in the quantum-enhanced feature spaces. It provides the encoding phase to map the real data and Boltzmann weight onto the quantum feature spaces and the training phase to learn an optimal inference function.  Specifically, the training phase provides a physical quantity to measure the posterior distribution in quantum feature spaces, and this measure is utilized to design the quantum maximum a posterior (QMAP) algorithm and the quantum predictive distribution estimator (QPDE). 

\item arXiv:1907.09965\\
Quantum Simulated Annealing for Bayesian Inference and Estimating Partition Functions\\
Authors propose a quantum simulated annealing algorithm for speeding up simulated annealing algorithms, where the stationary distributions of the Markov chains are Gibbs distributions at temperatures specified according to an annealing schedule. It is then applied to estimating partition functions and Bayesian inference.  

\item arXiv:1904.06166\\
Adaptive Bayesian phase estimation for quantum error correcting codes\\
Authors show how to use Bayesian inference to determine phase shifts of multi-qubit states. The method allows for the selection of an adaptive basis for the measurements. It can also process the outcomes of different observables at the same time. The method leads to a substantial decrease in the resources needed, speeds up the state characterisation and optimisation in experimental implementations.

\item arXiv:2110.10378\\
Machine Learning for Continuous Quantum Error Correction on Superconducting Qubits\\
Authors proposes a RNN based continuous QECC scheme to identity bit-flip errors from continuous noisy syndrome measurements. It operates on measurement signals deviating from the ideal behavior in which the mean value corresponds to a code syndrome value and the measurement has white noise. Three noise cases are studied: auto-correlation at temporal short lags, transient syndrome dynamics after each bit-flip, and drift in the steady-state syndrome values over the course of many experiments.

\item arXiv:1812.08862\\
Training of Quantum Circuits on a Hybrid Quantum Computer\\
Authors implement a quantum circuit training algorithm on the canonical Bars-and-Stripes data set. They use two separate strategies: Particle Swarm and Bayesian optimization and show that the convergence to the target distribution depends critically on both the quantum hardware and classical optimization strategy.

\item arXiv:1812.04877\\
Quantum Statistical Inference\\
Thesis the covers: (1) training of quantum Gaussian processes (2) a novel algorithm for solving linear systems (3) task of encoding the classical data into a quantum state for machine learning applications (4) apply the quantum enhanced GPs to Bayesian deep learning (5) analytical toolkit for causal inference in quantum data (6) connection between causality and quantum communications (7) general bound for the quantum capacity of noisy communication channels.

\item arXiv:1809.05072\\
A controlled-NOT gate for frequency-bin qubits\\
In this article, they design and implement the first entangling gate for frequency-bin qubits, a coincidence-basis controlled-NOT (CNOT). They use a novel parameter inference approach based on Bayesian machine learning, which enables accurate gate reconstruction from measurements in the two-photon computational basis alone. Their CNOT imparts a single-photon frequency shift controlled by the frequency of another photon.

\item arXiv:1806.11463\\
Bayesian Deep Learning on a Quantum Computer\\
Extending the Bayesian approach to deep architectures has remained a major challenge. Recent results connected deep feedforward neural networks with Gaussian processes, allowing training without backpropagation. This connection enables the authors to leverage a quantum algorithm designed for Gaussian processes and develop a new algorithm for Bayesian deep learning on quantum computers. The properties of the kernel matrix in the Gaussian process ensure the efficient execution of the core component of the protocol, quantum matrix inversion, providing an at least polynomial speedup over classical algorithms.

\item arXiv:1805.11089\\
Bayesian Quantum Circuit\\
Parameterized quantum circuits (PQCs)

\item arXiv:1409.1524\\
Quantum Bootstrapping via Compressed Quantum Hamiltonian Learning\\
Authors show a new application for small quantum computers: characterizing and controlling larger quantum computers. In particular, how small quantum simulators can be used to characterize and learn control models for larger devices for wide classes of physically realistic Hamiltonians. They use Bayesian inference in concert with Lieb-Robinson bounds and interactive quantum learning methods to achieve compressed simulations for characterization. 

\item arXiv:0811.1792\\
Use of a Quantum Computer to do Importance and Metropolis-Hastings Sampling of a Classical Bayesian Network\\
Authors propose methods for doing importance sampling and Metropolis-Hastings sampling of a classical Bayesian network on a quantum computer.

\item arXiv:0511216\\
Bayesian updating of a probability distribution encoded on a quantum register\\
The updating procedure takes the form of a quantum algorithm that prepares the quantum register in the state representing the posterior distribution.

\item arXiv:0004028\\
Quantum Computer as a Probabilistic Inference Engine\\
Authors propose a new class of algorithms which generalize many standard ones. The goal of our algorithms is to estimate probability distributions. Such estimates are useful in, for example, applications of Decision Theory and Artificial Intelligence, where inferences are made based on uncertain knowledge.

\end{enumerate}
\section{Error mitigation}
\subsection{PEC}
\subsection{ZNE}
\subsection{Approximate QEC}
\subsection{Channel adaptive QEC}
\subsection{Clifford data regression}

\added{
% Work related to QEM
% Probabilistic error cancellation
The paper \cite{van2023probabilistic} discusses a practical protocol for mitigating noise in noisy quantum computers, specifically addressing the challenges of learning and inverting a sparse noise model that captures correlated errors. The protocol, called probabilistic error cancellation (PEC), enables the removal of noise-induced biases in high-weight observables across the full circuit. The approach relies on accurate noise representation, efficient learning, and an effective noise-inversion scheme. The protocol has been demonstrated on a superconducting quantum processor with crosstalk errors, providing an important milestone towards achieving noise-free observables in larger quantum circuits. The results validate the accuracy, efficiency, and scalability of the learning protocol and highlight its potential as a characterization and benchmarking tool for studying and mitigating noise in quantum processors.
% NISQ algorithms and QEM review
NISQ devices, although not error-corrected, have shown promise in various applications across different disciplines. The paper \cite{bharti2022noisy} highlights the need for accurate certification and verification of the outputs of NISQ computers, as they are crucial for assessing the reliability and stability of these devices. It mentions the challenges in achieving fault-tolerant quantum computing with millions of qubits and low error rates, which may take decades of research. However, in the meantime, the focus is on maximizing the computational power of current NISQ devices and developing techniques to mitigate errors. The paper emphasizes the importance of algorithm design and application-specific problems to harness the potential of NISQ devices.
}
%
\section{Information theory}
% Work related to Information theory
% Toth: Quantum metrology from a quantum information science perspective
\added{
The paper \cite{toth2014quantum} covers various aspects of quantum metrology, including simple metrological setups and fundamental concepts such as shot-noise scaling, Heisenberg scaling, quantum Fisher information, and the Cramer-Rao bound. The authors demonstrate that entanglement is necessary to surpass the shot-noise scaling in metrological tasks with linear interferometers. They explore applications of quantum Fisher information and its relation to macroscopic superpositions, the speed of quantum evolution, and the quantum Zeno effect. The paper also addresses the impact of uncorrelated noise on the achievable precision in metrological tasks, highlighting the connection to the survival of multipartite entanglement in noisy environments. It emphasizes the role of entanglement in improving the precision of quantum measurements and the implications of noise on metrological scalability.
% Learning theory preskill
The paper \cite{huang2022foundations} explores the problem of learning physical operations in a quantum machine from experiments, considering both the intrinsic descriptions of the operations and the ability to predict the extrinsic behavior of the quantum system. The authors use a learning-theoretic perspective and present results on what can and cannot be learned from noisy quantum experiments. They distinguish between learning the intrinsic descriptions of the operations and predicting the experimental outcomes. The paper provides fundamental results on the learnability of noise models in quantum systems and demonstrates a polynomial quantum advantage in a learning task using noisy quantum devices. The authors also discuss future directions, including the clarification of learnable and unlearnable model classes and the possibility of engineering quantum systems to facilitate learning. Ultimately, the paper aims to deepen our understanding of what can be learned from quantum experiments and its implications for quantum technology and our knowledge of the physical world.
}
\section{Key challenges}
% by the end of this section, reader should have a technical understanding of the research question
%Device level composite reliability does not exist even though DiVincenzo starts the discussion here: the minimum requirements for the physical implementation of quantum computation here \added{divincenzo2000physical}. These metrics correspond to the minimum requirements for the physical implementation of quantum computing, which fall into one of the five classes: SPAM (state preparation and measurement) fidelity, single-qubit gate fidelity, two-qubit entangling gate fidelity, duty cycle (gate length to coherence time ratio), and addressability (ability to measure a register element without interference from other qubits).
Several key takeaways emerged from the analysis in this chapter. Firstly, despite various terminologies used for measuring output quality in noisy quantum computers, statistical taxonomy including terms such as computational accuracy, result reproducibility, output stability, and device reliability, lack clear definitions and distinctions. This gap in research necessitates further exploration and clarification. Furthermore, though databases of quantum noise characterization data are publicly accessible from certain vendors such as IBM alongwith device characterization studies, a comprehensive investigation and characterization of the non-stationarity of quantum noise, particularly in transmon architectures, remain unexplored. This highlights the need to address the devices' temporal and spatial variability, leading to device reliability challenges. Thirdly, although ample characterization data is available, its systematic utilization for estimating performance bounds on program output remains unclear. Bridging this gap requires attention to developing methods for effective estimation using characterization data rather than relying solely on experiments. Fourthly, the literature features numerous mitigation algorithms, but there is a demand for adaptive algorithms that can handle the adverse effects of time-varying quantum noise. Further exploration and development of such algorithms are necessary. Lastly, understanding the trade-offs between output stability, accuracy, and reproducibility when utilizing unreliable devices is crucial. The absence of quantum analogues to classical bias-variance trade-offs calls for a deeper exploration of trade-offs in real-time estimation and execution of dynamic mitigation circuits, such as probabilistic error cancellation. 

\par This research study addresses the question of defining and distinguishing computational accuracy, result reproducibility, output stability, and device reliability in the presence of spatio-temporal non-stationarity of quantum registers. The research will delve into characterizing spatial and temporal differences in noise statistics, estimating performance limits using characterization data, employing adaptive algorithms to mitigate time-varying quantum noise, and comprehending the trade-offs in optimizing output stability, accuracy, and reproducibility with unreliable devices.
